Do LLMs "know" internally when they follow instructions?

Instruction-following is crucial for building AI agents with large language models (LLMs), as these models must adhere strictly to user-provided constraints and guidelines. However, LLMs often fail to follow even simple and clear instructions. To improve instruction-following behavior and prevent undesirable outputs, a deeper understanding of how LLMs' internal states relate to these outcomes is required. In this work, we investigate whether LLMs encode information in their representations that correlate with instruction-following success - a property we term knowing internally. Our analysis identifies a direction in the input embedding space, termed the instruction-following dimension, that predicts whether a response will comply with a given instruction. We find that this dimension generalizes well across unseen tasks but not across unseen instruction types. We demonstrate that modifying representations along this dimension improves instruction-following success rates compared to random changes, without compromising response quality. Further investigation reveals that this dimension is more closely related to the phrasing of prompts rather than the inherent difficulty of the task or instructions. This work provides insight into the internal workings of LLMs' instruction-following, paving the way for reliable LLM agents.

==> contents/conclusion.tex <==
\section{Conclusion}
% \textbf{Summary-contribution}
We analyzed instruction-following in LLMs, and found that the internal state of LLMs can be used to infer instruction following while generalizing across tasks.  Using representation engineering, we identified a  key dimension within the input embedding space linked to successful instruction-following. This dimension generalized to unseen tasks, we showed that using this dimension with representation engineering can boost instruction-following success rates without sacrificing response quality.

Furthermore, investigation of the impact of tokens and layers on separability and analysis of the similarity between the identified direction and directions due to known perturbations shows that this dimension is more related to the rephrasing of prompts rather than the inherent difficulty of the task or instructions.  Our findings highlight the crucial role of prompt encoding in instruction-following success for LLMs. The sensitivity of the input embedding space to slight changes in phrasing explains why LLMs may fail to follow even clear instructions and why prompt engineering is effective. By adjusting the representations directly, as we did with representation engineering, we show that it is possible to significantly improve instruction adherence. Going forward, improving the robustness of LLMs' input embeddings through training can make models more reliable and consistent in following instructions across a variety of tasks. This is crucial for building trustworthy AI systems, especially in real-world applications where accuracy and reliability are essential.

% \juyeon{Need update}  Our findings also provide new insights into the importance of prompt encoding, offering an explanation for why LLMs sometimes fail to follow clear instructions and why prompt engineering can effectively influence model behavior.


% We explored instruction-following in LLMs, identifying a key dimension within the input embedding space linked to successful instruction-following. This dimension generalizes to unseen tasks, and representation engineering can leverage it to boost success rates without sacrificing response quality. 
% While our work enhances LLM instruction-following, it could potentially be misused to improve the generation of misleading or harmful content.

% In this work, we explored the challenge of instruction-following in LLMs by analyzing the internal representations that differentiate success from failure cases. Our key contribution is the observation of a specific dimension within the input embedding space that is closely associated with successful instruction-following. We demonstrated that this dimension is generalizable to unseen tasks and can be leveraged through representation engineering to enhance the success rate of instruction-following, without compromising response quality.






\textbf{Limitations and Future work}
Our analysis was primarily focused on a specific set of tasks and models. Although our current results are consistent across the models we studied, future work could benefit from exploring additional models to ensure the robustness of the identified dimension across different LLM contexts. Additionally, expanding the dataset to include a wider variety of instruction-following cases could enrich the analysis and improve the generalizability of our findings.  We focused our investigation on simple modeling approaches to identify an instruction-following dimension and evaluate its practical significance.
Future work could include additional methods train linear probes, particularly in handling domain shifts. 
% Exploring more robust methods for probe training could enhance the accuracy and reliability of our findings. 
Similarly, better approaches to representation engineering \citep{zou2023representation} could further improve the success rate of instruction-following modifications.
Finally, unambiguously interpreting the meaning of the instruction-following dimension remains an open question. We considered three hypotheses and found that phrasing modification was most closely related to the dimension associated with instruction-following using a perturbation-based approach.  Additional investigations to develop systematic approaches to interpret the dimension could add to a deeper understanding of its meaning and implications.   
% However, there may be other interpretations of this dimension that we have yet to consider. 
Future research could develop systematic approaches to uncover the full meaning and implications of this dimension.

% In conclusion, our work contributes to the understanding of instruction-following in LLMs, revealing new dimensions of analysis and paving the way for future research to build on these insights.

% \textbf{Broader impacts}
% While our findings advance the understanding of LLM behavior, there is a potential risk that enhancing instruction-following capabilities could be exploited to create more convincing disinformation or other malicious content. However, this work primarily focuses on foundational research, and the broader societal impacts would largely depend on how these capabilities are applied in specific contexts.





% \section{Conclusion}

% \textbf{Summary-contribution}

% \textbf{Limitations and Futurework}
% More domains/models/.
% More analysis in Interpreting the meaning of the instruction-following dimensions.
% Better ways to train linear probes: maybe better with domain shift problems.
% Better methods for Representation engineering, such as projection, ...
% More instruction-following data
% More models: by size, more layers, tracking by tokens,…
% (So far, results are consistent, so we don’t need more model for this project)









==> contents/ifeval_simple_data_generation.tex <==
\subsection{Data generation}

We collect Representations when Generation(RwG). We use the first token, last part. However, IFEval data includes multiple tasks for each instruction type, which can leading to find mixed dimensions of different task and instruction-following. Thus, we generate IFEval-simple with fixed 20 tasks for 23 instructions, total 460 data points. 

Also,  Big category: keyword:frequency, keyword:existence, keyword:forbidden\_words, detectable-format:constrained\_response, detectable\_content:number\_placeholders, startend:end\_checker,  Sub category: include 102 different types of sub category e.g., keyword:frequency — elephant three times, coffee 10 times, ... Task: 102 task And retry instruction generalization again. I don’t need to use whole instructions in the IFEval data. Punctuation is useless in building Agent AI.  Also in the simple IFEval I made, only one types of inst is included. Train on keyword and test on detectble-format. Might be work.

\input{contents/table/ifeval_simple_0706_success_rate}

==> contents/last_figure_page.tex <==


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{iclr2024//contents//figures//RE/RE_example.png}
%     \caption{\textbf{RE example} An illustrative example of modified responses. In this case, the task was to write a resume with the instruction to include three specific keywords. The original response only included one keyword, whereas the modified response, guided by the instruction-following direction, successfully incorporated all three keywords, demonstrating the effectiveness of RE in enhancing instruction adherence.}
%     \label{fig:RE_example}
% \end{figure}




==> contents/milestones.tex <==
\section*{Milestones}
\subsection{Write skeleton: one for a day}
\begin{itemize}
    \item \sout{Tue: Generate experiment tables}
    \item \sout{Tue: Write introduction skeleton + contributions (sec 1)}
    \item \sout{Thu: Make pretty figures}
    \item \sout{5: Write RwG skeleton (sec 2) + Write RE skeleton (sec 3) + Write Discussion skeleton (sec 4)}
    \item 7: Write Discussion \& Related work \& Conclusion skeleton (sec 4, 5, 6)
\end{itemize}

\subsection{Write draft: one for a day}
\begin{itemize}
    \item 11: Write introduction draft + contributions (sec 1)
    \item 12: Write RwG draft (sec 2) \& Draw Figure 1 \& Write RE draft (sec 3)
    \item 13: Write Discussion draft (sec 4)
    \item 14: Write Related work \& Conclusion draft (sec 5, 6)
    \item 15: polish figures
\end{itemize}

\subsection{Share: Jaya, Chritina, Shierly}

\subsection{Polishing draft: one for a day}
\begin{itemize}
    \item 16: Write RwG polish (sec 2)
    \item 17: Write RE polish (sec 3)
    \item 18: Write Discussion polish (sec 4) 
    \item 21: sec 3
    \item 22: related work
\end{itemize}

\subsection{Share: Jaya, Chritina, Shierly and others}

\subsection{Refinement: one for a day}
\begin{itemize}
    \item 21: Write RwG Refinement (sec 2) + Write RE Refinement (sec 3)
    \item 22: Write Discussion Refinement (sec 4)
    \item 23: Write Related work \& Conclusion Refinement (sec 5, 6)
    \item 24: Write introduction Refinement + contributions (sec 1)
    \item 25: Refine Appendix
\end{itemize}


\subsection{Submit Apple internal}

==> contents/table/RE_filter.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lllll@{}}
% \toprule
%         & ori success rate & random success rate & normal success rate & detect\_ratio(TN/TN+FN) & random F2T/(F2T+F2F) & normal F2T/(F2T+F2F) & random T2T/(T2T+T2F) & normal T2T/(T2T+T2F) \\ \midrule
% keywords:forbidden\_words                & 0.15686          & 0.15686             & 0.17647             & 1                       & 0.09302              & 0.09302              & 0.5                  & 0.625                \\
% keywords:existence                       & 0.78431          & 0.78431             & 0.80392             & 1                       & 0.27273              & 0.31818              & 0.925                & 0.9375               \\
% keywords:frequency                       & 0.85294          & 0.79412             & 0.89216             & 1                       & 0.42857              & 0.66667              & 0.85227              & 0.93103              \\
% detectable\_content:number\_placeholders & 0.63726          & 0.68628             & 0.69608             & 1                       & 0.37838              & 0.37838              & 0.86154              & 0.87692              \\
% startend:end\_checker                    & 0.23529          & 0.18628             & 0.18628             & 1                       & 0.12821              & 0.10256              & 0.375                & 0.45833              \\
% Average                                  & 0.53333          & 0.52157             & 0.55098             & 1                       & 0.26018              & 0.31176              & 0.70276              & 0.76576   \\           
% \bottomrule
% \end{tabular}
% }
% \caption{7B model, last layer,alpha select using the validation set for each instruction, threshold=0.6, only high quality answers(over 8 scores)}
% \label{tab:RE_all_filter}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lllll@{}}
% \toprule
%         & ori success rate & random success rate & normal success rate & detect\_ratio(TN/TN+FN) & random F2T/(F2T+F2F) & normal F2T/(F2T+F2F) & random T2T/(T2T+T2F) & normal T2T/(T2T+T2F) \\ \midrule
% keywords:forbidden\_words                & 0.23529                              & 0.22549                                 & 0.27451                                 & 0.64103                                     & 0.02564                                  & 0.10256                                  & 0.83333                                  & 0.875                                    \\
% keywords:existence                       & 0.69608                              & 0.66667                                 & 0.69608                                 & 0.35484                                     & 0.06452                                  & 0.03226                                  & 0.92958                                  & 0.98592                                  \\
% keywords:frequency                       & 0.85294                              & 0.82353                                 & 0.85294                                 & 0.13333                                     & 0                                        & 0                                        & 0.96552                                  & 1                                        \\
% detectable\_content:number\_placeholders & 0.70588                              & 0.66667                                 & 0.71569                                 & 0.13333                                     & 0.03125                                  & 0.06667                                  & 0.95714                                  & 0.98611                                  \\
% startend:end\_checker                    & 0.30392                              & 0.33333                                 & 0.32353                                 & 0.59155                                     & 0.11268                                  & 0.07042                                  & 0.83871                                  & 0.90323                                  \\
% Average                                  & 0.55882                              & 0.54314                                 & 0.57255                                 & 0.37082       & 0.04682                                  & 0.05438                                  & 0.90486  \\           
% \bottomrule
% \end{tabular}
% }
% \caption{13B model, last layer,alpha select using the validation set for each instruction, threshold=0.6, only high quality answers(over 8 scores)}
% \label{tab:RE_all_filter}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lllll@{}}
% \toprule
%         & ori success rate & random success rate & normal success rate & detect\_ratio(TN/TN+FN) & random F2T/(F2T+F2F) & normal F2T/(F2T+F2F) & random T2T/(T2T+T2F) & normal T2T/(T2T+T2F) \\ \midrule
%         keywords:forbidden\_words                & 0.23529                              & 0.2351                                  & 0.23529                                 & 0.84615                                     & 0.03846                                  & 0.02564                                  & 0.90666                                  & 0.91667                                  \\
% keywords:existence                       & 0.68628                              & 0.69608                                 & 0.71569                                 & 0.625                                       & 0.0625                                   & 0.15625                                  & 0.98571                                  & 0.97143                                  \\
% keywords:frequency                       & 0.84314                              & 0.84314                                 & 0.86275                                 & 0.9375                                      & 0.25                                     & 0.375                                    & 0.95349                                  & 0.95349                                  \\
% detectable\_content:number\_placeholders & 0.36275                              & 0.36275                                 & 0.41177                                 & 0.83077                                     & 0.15385                                  & 0.15385                                  & 0.72973                                  & 0.86487                                  \\
% startend:end\_checker                    & 0.64706                              & 0.60784                                 & 0.64706                                 & 0.77778                                     & 0.22222                                  & 0.11111                                  & 0.81818                                  & 0.93939                                  \\
% Average                                  & 0.5549                               & 0.54898                                 & 0.57451                                 & 0.80344                                     & 0.14541                                  & 0.16437                                  & 0.87875                                  & 0.92917      \\           
% \bottomrule
% \end{tabular}
% }
% \caption{Mistral model, last layer,alpha select using the validation set for each instruction, threshold=0.6, only high quality answers(over 8 scores)}
% \label{tab:RE_all_filter}
% \end{table}



% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lllll@{}}
% \toprule
%         & ori success rate & random success rate & normal success rate & detect\_ratio(TN/TN+FN) & random F2T/(F2T+F2F) & normal F2T/(F2T+F2F) & random T2T/(T2T+T2F) & normal T2T/(T2T+T2F) \\ \midrule
% keywords:forbidden\_words                & 0.10784                              & 0.15686                                 & 0.20588                                 & 0.96703                                     & 0.10989                                  & 0.12088                                  & 0.54546                                  & 0.90909                                  \\
% keywords:existence                       & 0.77451                              & 0.68628                                 & 0.79412                                 & 0.91304                                     & 0.30435                                  & 0.46154                                  & 0.8052                                   & 0.91139                                  \\
% keywords:frequency                       & 0.84314                              & 0.70115                                 & 0.89216                                 & 0.8125                                      & 0.38889                                  & 0.42105                                  & 0.78947                                  & 0.98837                                  \\
% detectable\_content:number\_placeholders & 0.47059                              & 0.48039                                 & 0.48039                                 & 0.92593                                     & 0.30357                                  & 0.25926                                  & 0.69565                                  & 0.72917                                  \\
% startend:end\_checker                    & 0.26471                              & 0.26471                                 & 0.35294                                 & 1                                           & 0.16                                     & 0.24                                     & 0.55556                                  & 0.66667                                  \\
% Average                                  & 0.49216                              & 0.45788                                 & 0.5451                                  & 0.9237                                      & 0.25334                                  & 0.30055                                  & 0.67827                                  & 0.84094                                 
%  \\           
% \bottomrule
% \end{tabular}
% }
% \caption{Phi3 model, last layer,alpha select using the validation set for each instruction, threshold=0.6, only high quality answers(over 8 scores)}
% \label{tab:RE_all_filter}
% \end{table}





% ----------------------------------
% \begin{table}[h!]
% \resizebox{\columnwidth}{!}{%
% \centering
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Model} & \textbf{Original SR} & \textbf{Random SR} & \textbf{Inst-f SR} & \textbf{Detect Ratio} & \textbf{Random F2T} & \textbf{Inst-f F2T} & \textbf{Random T2T} & \textbf{Inst-f T2T} \\
% \midrule
% \textbf{7b model} & & & & & & & & \\
% keywords:forbidden\_words & 0.16 & 0.16 & 0.18 & 1.00 & 0.09 & 0.09 & 0.50 & 0.63 \\
% keywords:existence & 0.78 & 0.78 & 0.80 & 1.00 & 0.27 & 0.32 & 0.93 & 0.94 \\
% keywords:frequency & 0.85 & 0.79 & 0.89 & 1.00 & 0.43 & 0.67 & 0.85 & 0.93 \\
% detectable\_content:number\_placeholders & 0.64 & 0.69 & 0.70 & 1.00 & 0.38 & 0.38 & 0.86 & 0.88 \\
% startend:end\_checker & 0.24 & 0.19 & 0.19 & 1.00 & 0.13 & 0.10 & 0.38 & 0.46 \\\midrule
% Average & 0.53 & 0.52 & 0.55 & 1.00 & 0.26 & 0.31 & 0.70 & 0.77 \\
% \midrule
% \textbf{13b model} & & & & & & & & \\
% keywords:forbidden\_words & 0.24 & 0.23 & 0.27 & 0.64 & 0.03 & 0.10 & 0.83 & 0.88 \\
% keywords:existence & 0.70 & 0.67 & 0.70 & 0.35 & 0.06 & 0.03 & 0.93 & 0.99 \\
% keywords:frequency & 0.85 & 0.82 & 0.85 & 0.13 & 0.00 & 0.00 & 0.97 & 1.00 \\
% detectable\_content:number\_placeholders & 0.71 & 0.67 & 0.72 & 0.13 & 0.03 & 0.07 & 0.96 & 0.99 \\
% startend:end\_checker & 0.17 & 0.22 & 0.26 & 0.67 & 0.06 & 0.12 & 1.00 & 1.00 \\\midrule
% Average & 0.53 & 0.52 & 0.56 & 0.39 & 0.04 & 0.06 & 0.94 & 0.97 \\
% \midrule
% \textbf{Phi3 model} & & & & & & & & \\
% keywords:forbidden\_words & 0.11 & 0.16 & 0.21 & 0.97 & 0.11 & 0.12 & 0.55 & 0.91 \\
% keywords:existence & 0.77 & 0.69 & 0.79 & 0.91 & 0.30 & 0.46 & 0.81 & 0.91 \\
% keywords:frequency & 0.84 & 0.70 & 0.89 & 0.81 & 0.39 & 0.42 & 0.79 & 0.99 \\
% detectable\_content:number\_placeholders & 0.47 & 0.48 & 0.48 & 0.93 & 0.30 & 0.26 & 0.70 & 0.73 \\
% startend:end\_checker & 0.14 & 0.16 & 0.22 & 1.00 & 0.08 & 0.18 & 0.43 & 0.64 \\\midrule
% Average & 0.47 & 0.44 & 0.52 & 0.92 & 0.24 & 0.29 & 0.65 & 0.84 \\
% \midrule
% \textbf{Mistral model} & & & & & & & & \\
% keywords:forbidden\_words & 0.36 & 0.41 & 0.50 & 1.00 & 0.13 & 0.25 & 1.00 & 1.00 \\
% keywords:existence & 0.79 & 0.81 & 0.86 & 0.67 & 0.14 & 0.33 & 1.00 & 1.00 \\
% keywords:frequency & 0.86 & 0.89 & 0.90 & 0.64 & 0.15 & 0.29 & 1.00 & 1.00 \\
% detectable\_content:number\_placeholders & 0.36 & 0.36 & 0.41 & 0.83 & 0.15 & 0.15 & 0.73 & 0.86 \\
% startend:end\_checker & 0.25 & 0.28 & 0.35 & 0.97 & 0.07 & 0.13 & 1.00 & 1.00 \\\midrule
% Average & 0.53 & 0.55 & 0.61 & 0.82 & 0.13 & 0.23 & 0.95 & 0.97 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Success Rates, Detect Ratios, and F2T/T2T Ratios across Models, only high quality answers(over 8 scores)}
% \label{tab:models2}
% \end{table}



\begin{table}[H]
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} & \textbf{Original SR} & \textbf{Inst-f SR} & \textbf{Random SR} & \textbf{Detect Ratio} & \textbf{Inst-f F2T} & \textbf{Random F2T} & \textbf{Inst-f T2T} & \textbf{Random T2T} \\
\midrule
\textbf{7b model} & & & & & & & & \\
keywords:forbidden\_words & 0.16 & 0.18 & 0.16 & 1.00 & 0.09 & 0.09 & 0.63 & 0.50 \\
keywords:existence & 0.78 & 0.80 & 0.78 & 1.00 & 0.32 & 0.27 & 0.94 & 0.93 \\
keywords:frequency & 0.85 & 0.89 & 0.79 & 1.00 & 0.67 & 0.43 & 0.93 & 0.85 \\
detectable\_content:number\_placeholders & 0.64 & 0.70 & 0.69 & 1.00 & 0.38 & 0.38 & 0.88 & 0.86 \\
startend:end\_checker & 0.24 & 0.19 & 0.19 & 1.00 & 0.10 & 0.13 & 0.46 & 0.38 \\\midrule
Average & 0.53 & 0.55 & 0.52 & 1.00 & 0.31 & 0.26 & 0.77 & 0.70 \\
\midrule
\textbf{13b model} & & & & & & & & \\
keywords:forbidden\_words & 0.24 & 0.27 & 0.23 & 0.64 & 0.10 & 0.03 & 0.88 & 0.83 \\
keywords:existence & 0.70 & 0.70 & 0.67 & 0.35 & 0.03 & 0.06 & 0.99 & 0.93 \\
keywords:frequency & 0.85 & 0.85 & 0.82 & 0.13 & 0.00 & 0.00 & 1.00 & 0.97 \\
detectable\_content:number\_placeholders & 0.71 & 0.72 & 0.67 & 0.13 & 0.07 & 0.03 & 0.99 & 0.96 \\
startend:end\_checker & 0.17 & 0.26 & 0.22 & 0.67 & 0.12 & 0.06 & 1.00 & 1.00 \\\midrule
Average & 0.53 & 0.56 & 0.52 & 0.39 & 0.06 & 0.04 & 0.97 & 0.94 \\
\midrule
\textbf{Mistral model} & & & & & & & & \\
keywords:forbidden\_words & 0.36 & 0.50 & 0.37 & 1.00 & 0.25 & 0.13 & 1.00 & 1.00 \\
keywords:existence & 0.79 & 0.86 & 0.81 & 0.67 & 0.33 & 0.14 & 1.00 & 1.00 \\
keywords:frequency & 0.86 & 0.90 & 0.89 & 0.64 & 0.29 & 0.15 & 1.00 & 1.00 \\
detectable\_content:number\_placeholders & 0.36 & 0.41 & 0.36 & 0.83 & 0.15 & 0.15 & 0.86 & 0.73 \\
startend:end\_checker & 0.25 & 0.35 & 0.28 & 0.97 & 0.13 & 0.07 & 1.00 & 1.00 \\\midrule
Average & 0.52 & 0.60 & 0.54 & 0.82 & 0.23 & 0.13 & 0.97 & 0.95 \\
\midrule
\textbf{Phi3 model} & & & & & & & & \\
keywords:forbidden\_words & 0.11 & 0.21 & 0.16 & 0.97 & 0.12 & 0.11 & 0.91 & 0.55 \\
keywords:existence & 0.77 & 0.79 & 0.69 & 0.91 & 0.46 & 0.30 & 0.91 & 0.81 \\
keywords:frequency & 0.84 & 0.89 & 0.70 & 0.81 & 0.42 & 0.39 & 0.99 & 0.79 \\
detectable\_content:number\_placeholders & 0.47 & 0.48 & 0.48 & 0.93 & 0.26 & 0.30 & 0.73 & 0.70 \\
startend:end\_checker & 0.14 & 0.22 & 0.16 & 1.00 & 0.18 & 0.08 & 0.64 & 0.43 \\\midrule
Average & 0.47 & 0.52 & 0.44 & 0.92 & 0.29 & 0.24 & 0.84 & 0.65 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Transition metrics for Representation Engineering on the last layer across four models}.
This table shows the success rate (SR) for high-quality responses in task execution, focusing on False-to-True (F2T) and True-to-True (T2T) transitions. The detect ratio represents the proportion of failure cases (20\% of the test set) identified by linear probes trained on the training set (70\%) and validated on the validation set (10\%), using a threshold selected on the validation set. Results demonstrate that RE using the instruction-following dimension consistently improves success rates across instruction types, with higher F2T and T2T values compared to random directions.}
\label{tab:RE_filter}
\end{table}




==> contents/table/RE_nonfilter.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lll@{}}
% \toprule
%         & Original Success Rate & Random Success Rate & Normal Success Rate & Original quality raito & Random quality raito & Normal quality raito \\ \midrule
% keywords:forbidden\_words                & 0.18628               & 0.18628             & 0.20588             & 0.73684                & 0.73684              & 0.80952              \\
% keywords:existence                       & 0.79412               & 0.79412             & 0.81373             & 0.97531                & 0.93827              & 0.95181              \\
% keywords:frequency                       & 0.86275               & 0.81373             & 0.91177             & 0.88636                & 0.84337              & 0.86022              \\
% detectable\_content:number\_placeholders & 0.76471               & 0.79412             & 0.82353             & 0.60256                & 0.4881               & 0.64197              \\
% startend:end\_checker                    & 0.23529               & 0.18628             & 0.18628             & 0.83333                & 0.78947              & 0.78947              \\
% Average                                  & 0.56863               & 0.5549              & 0.58824             & 0.80688                & 0.75921              & 0.8106          \\            
% \bottomrule
% \end{tabular}
% }
% \caption{7B model, last layer,alpha select using the validation set for each instruction, threshold=0.6, quality ratio: among success response, ratio of 9 scores}
% \label{tab:RE_all_nonfilter}
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lll@{}}
% \toprule
%         & Original Success Rate & Random Success Rate & Normal Success Rate & Original quality raito & Random quality raito & Normal quality raito \\ \midrule
% keywords:forbidden\_words                & 0.28431                                   & 0.23529                                 & 0.31372                                 & 0.86207                                    & 0.91667                                  & 0.9375                                   \\
% keywords:existence                       & 0.87255                                   & 0.88235                                 & 0.88235                                 & 1                                          & 0.98889                                  & 1                                        \\
% keywords:frequency                       & 0.92157                                   & 0.91177                                 & 0.91177                                 & 0.95745                                    & 0.96774                                  & 0.96774                                  \\
% detectable\_content:number\_placeholders & 0.80392                                   & 0.87255                                 & 0.90196                                 & 0.80488                                    & 0.69663                                  & 0.80435                                  \\
% startend:end\_checker                    & 0.16667                                   & 0.13725                                 & 0.18628                                 & 1                                          & 1                                        & 1                                        \\
% Average                                  & 0.6098                                    & 0.60784                                 & 0.63922                                 & 0.92488                                    & 0.91399                                  & 0.94192                                  \\            
% \bottomrule
% \end{tabular}
% }
% \caption{13B model, last layer,alpha select using the validation set for each instruction, threshold=0.6, quality ratio: among success response, ratio of 9 scores}
% \label{tab:RE_all_nonfilter}
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lll@{}}
% \toprule
%         & Original Success Rate & Random Success Rate & Normal Success Rate & Original quality raito & Random quality raito & Normal quality raito \\ \midrule
% keywords:forbidden\_words                &                                           &                                         &                                         &                                            &                                          &                                          \\
% keywords:existence                       & 0.86275                                   & 0.82353                                 & 0.90196                                 & 0.98864                                    & 0.97619                                  & 0.98913                                  \\
% keywords:frequency                       &                                           &                                         &                                         &                                            &                                          &                                          \\
% detectable\_content:number\_placeholders & 0.5098                                    & 0.44118                                 & 0.51961                                 & 0.78846                                    & 0.95556                                  & 0.9434                                   \\
% startend:end\_checker                    & 0.27451                                   & 0.2451                                  & 0.30392                                 & 1                                          & 0.96                                     & 1                                        \\
% Average                                  \\         
% \bottomrule
% \end{tabular}
% }
% \caption{Mistral model, last layer,alpha select using the validation set for each instruction, threshold=0.6, quality ratio: among success response, ratio of 9 scores}
% \label{tab:RE_all_nonfilter}
% \end{table}



% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|lll|lll@{}}
% \toprule
%         & Original Success Rate & Random Success Rate & Normal Success Rate & Original quality raito & Random quality raito & Normal quality raito \\ \midrule
% keywords:forbidden\_words                &                                           &                                         &                                         &                                            &                                          &                                          \\
% keywords:existence                       & 0.94118                                   & 0.94118                                 & 0.98039                                 & 0.79167                                    & 0.75                                     & 0.84                                     \\
% keywords:frequency                       & 1                                         & 1                                       & 1                                       & 0.78431                                    & 0.69608                                  & 0.78431                                  \\
% detectable\_content:number\_placeholders &                                           &                                         &                                         &                                            &                                          &                                          \\
% startend:end\_checker                    & 0.13725                                   & 0.14706                                 & 0.17647                                 & 1                                          & 1                                        & 0.94444                                  \\
% Average                                  &                                           &                                         &                                         &                                            &                                          &     \\         
% \bottomrule
% \end{tabular}
% }
% \caption{Phi model, last layer,alpha select using the validation set for each instruction, threshold=0.6, quality ratio: among success response, ratio of 9 scores}
% \label{tab:RE_all_nonfilter}
% \end{table}

%--------------


% \begin{table}[h!]
% \resizebox{\columnwidth}{!}{%
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Model} & \textbf{Original SR} & \textbf{Random SR} & \textbf{Normal SR} & \textbf{Original QR} & \textbf{Random QR} & \textbf{Normal QR} \\
% \midrule
% \textbf{7b model} & & & & & & \\
% keywords:forbidden\_words & 0.19 & 0.19 & 0.21 & 0.74 & 0.74 & 0.81 \\
% keywords:existence & 0.79 & 0.79 & 0.81 & 0.98 & 0.94 & 0.95 \\
% keywords:frequency & 0.86 & 0.81 & 0.91 & 0.89 & 0.84 & 0.86 \\
% detectable\_content:number\_placeholders & 0.76 & 0.79 & 0.82 & 0.60 & 0.49 & 0.64 \\
% startend:end\_checker & 0.24 & 0.19 & 0.19 & 0.83 & 0.79 & 0.79 \\\midrule
% Average & 0.57 & 0.55 & 0.59 & 0.81 & 0.76 & 0.81 \\
% \midrule
% \textbf{13b model} & & & & & & \\
% keywords:forbidden\_words & 0.28 & 0.24 & 0.31 & 0.86 & 0.92 & 0.94 \\
% keywords:existence & 0.87 & 0.88 & 0.88 & 1.00 & 0.99 & 1.00 \\
% keywords:frequency & 0.92 & 0.91 & 0.91 & 0.96 & 0.97 & 0.97 \\
% detectable\_content:number\_placeholders & 0.80 & 0.87 & 0.90 & 0.80 & 0.70 & 0.80 \\
% startend:end\_checker & 0.17 & 0.14 & 0.19 & 1.00 & 1.00 & 1.00 \\\midrule
% Average & 0.61 & 0.61 & 0.64 & 0.92 & 0.91 & 0.94 \\
% \midrule
% \textbf{Mistral model} & & & & & & \\
% keywords:forbidden\_words & 0.36 & 0.35 & 0.50 & 1.00 & 0.89 & 1.00 \\
% keywords:existence & 0.86 & 0.82 & 0.90 & 0.99 & 0.98 & 0.99 \\
% keywords:frequency & 0.91 & 0.85 & 0.93 & 0.97 & 0.99 & 0.98 \\
% detectable\_content:number\_placeholders & 0.51 & 0.44 & 0.52 & 0.79 & 0.96 & 0.94 \\
% startend:end\_checker & 0.27 & 0.25 & 0.30 & 1.00 & 0.96 & 1.00 \\\midrule
% Average & 0.58 & 0.54 & 0.63 & 0.95 & 0.95 & 0.98 \\
% \midrule
% \textbf{Phi model} & & & & & & \\
% keywords:forbidden\_words & 0.32 & 0.26 & 0.34 & 0.67 & 0.70 & 0.66 \\
% keywords:existence & 0.94 & 0.90 & 0.98 & 0.81 & 0.83 & 0.84 \\
% keywords:frequency & 1.00 & 1.00 & 1.00 & 0.77 & 0.70 & 0.81 \\
% detectable\_content:number\_placeholders & 0.87 & 0.85 & 0.95 & 0.55 & 0.56 & 0.57 \\
% startend:end\_checker & 0.14 & 0.16 & 0.22 & 1.00 & 1.00 & 1.00 \\\midrule
% Average & 0.65 & 0.64 & 0.70 & 0.76 & 0.76 & 0.78 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Success Rates and Quality Ratios across Models}
% \label{tab:models}
% \end{table}




\begin{table}[H]
\resizebox{\columnwidth}{!}{%
\centering
\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \textbf{Original SR} & \textbf{Inst-following SR} & \textbf{Random SR} & \textbf{Original QR} & \textbf{Inst-following QR} & \textbf{Random QR} \\
\midrule
\textbf{7b model} & & & & & & \\
keywords:forbidden\_words & 0.19 & 0.21 & 0.19 & 0.74 & 0.81 & 0.74 \\
keywords:existence & 0.79 & 0.81 & 0.79 & 0.98 & 0.95 & 0.94 \\
keywords:frequency & 0.86 & 0.91 & 0.81 & 0.89 & 0.86 & 0.84 \\
detectable\_content:number\_placeholders & 0.76 & 0.82 & 0.79 & 0.60 & 0.64 & 0.49 \\
startend:end\_checker & 0.24 & 0.19 & 0.19 & 0.83 & 0.79 & 0.79 \\\midrule
Average & 0.57 & 0.59 & 0.55 & 0.81 & 0.81 & 0.76 \\
\midrule
\textbf{13b model} & & & & & & \\
keywords:forbidden\_words & 0.28 & 0.31 & 0.24 & 0.86 & 0.94 & 0.92 \\
keywords:existence & 0.87 & 0.88 & 0.88 & 1.00 & 1.00 & 0.99 \\
keywords:frequency & 0.92 & 0.91 & 0.91 & 0.96 & 0.97 & 0.97 \\
detectable\_content:number\_placeholders & 0.80 & 0.90 & 0.87 & 0.80 & 0.80 & 0.70 \\
startend:end\_checker & 0.17 & 0.26 & 0.22 & 1.00 & 1.00 & 1.00 \\\midrule
Average & 0.61 & 0.65 & 0.62 & 0.92 & 0.94 & 0.92 \\
\midrule
\textbf{Mistral model} & & & & & & \\
keywords:forbidden\_words & 0.36 & 0.50 & 0.39 & 1.00 & 1.00 & 0.89 \\
keywords:existence & 0.86 & 0.90 & 0.82 & 0.99 & 0.99 & 0.98 \\
keywords:frequency & 0.91 & 0.93 & 0.89 & 0.97 & 0.98 & 0.99 \\
detectable\_content:number\_placeholders & 0.51 & 0.52 & 0.44 & 0.79 & 0.94 & 0.96 \\
startend:end\_checker & 0.25 & 0.35 & 0.28 & 1.00 & 1.00 & 0.96 \\\midrule
Average & 0.58 & 0.64 & 0.56 & 0.95 & 0.98 & 0.96 \\
\midrule
\textbf{Phi model} & & & & & & \\
keywords:forbidden\_words & 0.32 & 0.34 & 0.26 & 0.67 & 0.66 & 0.70 \\
keywords:existence & 0.94 & 0.98 & 0.90 & 0.81 & 0.84 & 0.83 \\
keywords:frequency & 1.00 & 1.00 & 1.00 & 0.77 & 0.81 & 0.70 \\
detectable\_content:number\_placeholders & 0.87 & 0.95 & 0.85 & 0.55 & 0.57 & 0.56 \\
startend:end\_checker & 0.14 & 0.22 & 0.16 & 1.00 & 1.00 & 1.00 \\\midrule
Average & 0.65 & 0.70 & 0.63 & 0.76 & 0.78 & 0.76 \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Detailed Representation Engineering results on the last layer across four models by instruction type}.
This table shows the success rates (SR) and quality ratios (QR) for each instruction type across four LLMs, comparing the original outputs, outputs using the instruction-following dimension, and outputs using random directions. RE along the instruction-following dimension improves SR across most instruction types while maintaining or enhancing QR, unlike random adjustments, which often lead to lower SR and QR.}
\label{tab:RE_appendix_non_filter}
\end{table}




==> contents/table/instruction_generalization_tokens.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}l|llll|llll|llll|llll@{}}
% \toprule
% Leave one out AUROC, ifeval\_simple\_0706 & \multicolumn{4}{l|}{7b}    & \multicolumn{4}{l|}{13b}   & \multicolumn{4}{l|}{mistral} & \multicolumn{4}{l|}{Phi3}  \\ \midrule
% inst                                      & 14   & 20   & 26   & 32   & 16   & 24   & 32   & 40   & 14    & 20    & 26   & 32   & 14   & 20   & 26   & 32   \\ \midrule
% keywords:forbidden\_words                 & 0.52 & 0.51 & 0.54 & 0.56 & 0.45 & 0.45 & 0.44 & 0.44 & 0.44  & 0.41  & 0.42 & 0.46 & 0.52 & 0.54 & 0.55 & 0.53 \\
% keywords:existence                        & 0.50 & 0.50 & 0.51 & 0.51 & 0.67 & 0.68 & 0.67 & 0.66 & 0.55  & 0.50  & 0.49 & 0.50 & 0.63 & 0.67 & 0.68 & 0.68 \\
% keywords:frequency                        & 0.57 & 0.59 & 0.58 & 0.59 & 0.57 & 0.57 & 0.57 & 0.57 & 0.56  & 0.56  & 0.56 & 0.56 & -    & -    & -    & -    \\
% detectable\_content:number\_placeholders  & 0.56 & 0.54 & 0.53 & 0.52 & 0.58 & 0.58 & 0.55 & 0.54 & 0.50  & 0.49  & 0.49 & 0.50 & 0.50 & 0.53 & 0.48 & 0.46 \\
% startend:end\_checker                     & 0.48 & 0.46 & 0.45 & 0.47 & 0.55 & 0.57 & 0.56 & 0.56 & 0.44  & 0.42  & 0.44 & 0.45 & 0.55 & 0.59 & 0.59 & 0.57 \\ \midrule
% AVERAGE                                   & 0.52 & 0.52 & 0.52 & 0.53 & 0.56 & 0.57 & 0.56 & 0.55 & 0.50  & 0.48  & 0.48 & 0.49 & 0.55 & 0.58 & 0.57 & 0.56 \\ \bottomrule
% \end{tabular}
% }
% \label{tab:inst_generalization_tokens}
% \caption{AUROC instructions generalization on different tokens}
% \end{table}


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|lll|lll|lll|lll@{}}
\toprule
Leave one out AUROC & \multicolumn{3}{l|}{\textbf{7b}}    & \multicolumn{3}{l|}{\textbf{13b}}   & \multicolumn{3}{l|}{\textbf{Mistral}} & \multicolumn{3}{l}{\textbf{Phi3}}  \\ \midrule
\textbf{inst} & \textbf{first token} & \textbf{middle token} & \textbf{last token} & \textbf{first token} & \textbf{middle token} & \textbf{last token} & \textbf{first token} & \textbf{middle token} & \textbf{last token} & \textbf{early token} & \textbf{middle token} & \textbf{last token} \\ \midrule
\textbf{keywords:forbidden\_words} & 0.52 & 0.55 & 0.53 & 0.45 & 0.54 & 0.47 & 0.44 & 0.41 & 0.42 & 0.52 & 0.47 & 0.50 \\
\textbf{keywords:existence} & 0.50 & 0.55 & 0.52 & 0.67 & 0.71 & 0.55 & 0.55 & 0.53 & 0.55 & 0.63 & 0.43 & 0.48 \\
\textbf{keywords:frequency} & 0.57 & 0.58 & 0.61 & 0.57 & 0.53 & 0.56 & 0.56 & 0.55 & 0.50 & - & - & - \\
\textbf{detectable\_content:number\_placeholders} & 0.56 & 0.38 & 0.44 & 0.58 & 0.53 & 0.52 & 0.50 & 0.52 & 0.51 & 0.50 & 0.48 & 0.45 \\
\textbf{startend:end\_checker} & 0.48 & 0.43 & 0.49 & 0.55 & 0.56 & 0.56 & 0.44 & 0.53 & 0.59 & 0.55 & 0.51 & 0.54 \\
\textbf{AVERAGE} & 0.52 & 0.50 & 0.52 & 0.56 & 0.58 & 0.53 & 0.50 & 0.51 & 0.51 & 0.55 & 0.51 & 0.51 \\ \bottomrule
\end{tabular}
}
\caption{Leave one out AUROC scores across different models and layers for early, middle, and last tokens.}
\label{tab:leave_one_out_auroc}
\end{table}


==> contents/table/meaning_of_dim_prompt_example.tex <==
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc}
\toprule 
\textbf{} & \textbf{Original Task} & \textbf{Task Familiarity} & \textbf{Instruction Difficulty} & \textbf{Phrasing Modification} \\\midrule
\textbf{Task} & Writing a summary of software engineer jobs & Writing a CV for a software engineer & Unchanged & Write about software engineer jobs \\ 
\textbf{Inst} & \makecell{Do not include keywords:\\ coding, Python, computer, experience} & Unchanged & Do not include the keyword "coding" & \makecell{Without keywords: \\coding, Python, or computer} \\\bottomrule
\end{tabular}
}
\caption{Task and Instruction Variations with Different Modifications}
\label{tab:task_variations}
\end{table}

\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|p{4cm} p{4cm} p{4cm} p{4cm}}
\toprule 
& \textbf{Original Task} & \textbf{Task Familiarity} & \textbf{Instruction Difficulty} & \textbf{Phrasing Modification} \\\midrule
\textbf{Task} & Writing a summary of software engineer jobs & Writing a CV for a software engineer & Unchanged & Write about software engineer jobs \\ \midrule
\textbf{Inst} & Do not include keywords: coding, Python, computer, experience & Unchanged & Do not include the keyword "coding" & Without keywords: coding, Python, or computer \\
\bottomrule
\end{tabular}
}
\caption{Task and Instruction Variations with Different Modifications}
\label{tab:task_variations}
\end{table}


==> contents/table/task_generalization_middle_token.tex <==
% \begin{table}[]
% \centering
% \resizebox{0.5\columnwidth}{!}{%
% \begin{tabular}{@{}l|llll@{}}
% \toprule
% \textbf{} & \textbf{Early layers} & \textbf{Middle layers} & \textbf{Middle last layers} & \textbf{Last layers} \\ \midrule
% \textbf{7b}      & 0.55 $\pm$ 0.07 & 0.51 $\pm$ 0.04 & 0.52 $\pm$ 0.02 & 0.54 $\pm$ 0.02 \\
% \textbf{13b}     & 0.58 $\pm$ 0.06 & 0.56 $\pm$ 0.05 & 0.56 $\pm$ 0.06 & 0.79 $\pm$ 0.03 \\
% \textbf{mistral} & 0.54 $\pm$ 0.05 & 0.51 $\pm$ 0.03 & 0.49 $\pm$ 0.05 & 0.49 $\pm$ 0.04 \\
% \textbf{phi3}    & 0.56 $\pm$ 0.04 & 0.56 $\pm$ 0.03 & 0.54 $\pm$ 0.07 & 0.53 $\pm$ 0.03 \\ \bottomrule
% \end{tabular}
% }
% \caption{AUROC scores for Middle token across different models and layers.}
% \label{tab:middle_token_results}
% \end{table}



\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|lll|lll|lll|lll@{}}
\toprule
AUROC & \multicolumn{3}{l|}{\textbf{Early layers}}    & \multicolumn{3}{l|}{\textbf{Middle layers}}   & \multicolumn{3}{l|}{\textbf{Middle last layers}} & \multicolumn{3}{l}{\textbf{Last layers}}  \\ \midrule
\textbf{} & \textbf{first token} & \textbf{middle token} & \textbf{last token} & \textbf{first token} & \textbf{middle token} & \textbf{first token} & \textbf{first token} & \textbf{middle token} & \textbf{last token} & \textbf{first token} & \textbf{middle token} & \textbf{last token} \\ \midrule
\textbf{7b} & 0.77 $\pm$ 0.04 & 0.55 $\pm$ 0.07 & 0.73 $\pm$ 0.04 & 0.75 $\pm$ 0.05 & 0.51 $\pm$ 0.04 & 0.76 $\pm$ 0.04 & 0.79 $\pm$ 0.03 & 0.52 $\pm$ 0.02 & 0.75 $\pm$ 0.04 & 0.73 $\pm$ 0.03 & 0.54 $\pm$ 0.02 & 0.70 $\pm$ 0.02 \\
\textbf{13b} & 0.83 $\pm$ 0.03 & 0.58 $\pm$ 0.06 & 0.82 $\pm$ 0.03 & 0.81 $\pm$ 0.02 & 0.56 $\pm$ 0.05 & 0.80 $\pm$ 0.04 & 0.81 $\pm$ 0.03 & 0.56 $\pm$ 0.06 & 0.78 $\pm$ 0.04 & 0.78 $\pm$ 0.04 & 0.79 $\pm$ 0.03 & 0.49 $\pm$ 0.05 \\
\textbf{mistral} & 0.74 $\pm$ 0.02 & 0.54 $\pm$ 0.05 & 0.72 $\pm$ 0.04 & 0.71 $\pm$ 0.05 & 0.51 $\pm$ 0.03 & 0.67 $\pm$ 0.04 & 0.74 $\pm$ 0.02 & 0.49 $\pm$ 0.05 & 0.73 $\pm$ 0.03 & 0.71 $\pm$ 0.03 & 0.49 $\pm$ 0.04 & 0.70 $\pm$ 0.03 \\
\textbf{phi3} & 0.88 $\pm$ 0.03 & 0.56 $\pm$ 0.04 & 0.86 $\pm$ 0.03 & 0.85 $\pm$ 0.03 & 0.56 $\pm$ 0.03 & 0.83 $\pm$ 0.02 & 0.66 $\pm$ 0.03 & 0.54 $\pm$ 0.07 & 0.71 $\pm$ 0.03 & 0.65 $\pm$ 0.05 & 0.53 $\pm$ 0.03 & 0.63 $\pm$ 0.04 \\ \bottomrule
\end{tabular}
}
\caption{AUROC scores across different models and layers for first, middle, and last tokens.}
\label{tab:all_combined_results}
\end{table}

==> contents/table/task_generalization_tokens.tex <==
\begin{table}[]
\begin{tabular}{@{}l|llll@{}}
\toprule
\textbf{} & \textbf{Early layers} & \textbf{Middle layers} & \textbf{Middle last layers} & \textbf{Last layers} \\ \midrule
\textbf{7b} & 0.77 $\pm$ 0.04 & 0.73 $\pm$ 0.04 & 0.75 $\pm$ 0.05 & 0.76 $\pm$ 0.04 \\
\textbf{13b} & 0.83 $\pm$ 0.03 & 0.82 $\pm$ 0.03 & 0.81 $\pm$ 0.02 & 0.80 $\pm$ 0.04 \\
\textbf{mistral} & 0.74 $\pm$ 0.02 & 0.72 $\pm$ 0.04 & 0.71 $\pm$ 0.05 & 0.67 $\pm$ 0.04 \\
\textbf{phi3} & 0.88 $\pm$ 0.03 & 0.86 $\pm$ 0.03 & 0.85 $\pm$ 0.03 & 0.83 $\pm$ 0.02 \\ \bottomrule
\end{tabular}
\label{tab:task_generalization}
\caption{AUROC of Task generaliation: 5 inst(3 category) x 100 tasks)}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{@{}l|llll@{}}
\toprule
\textbf{} & \textbf{Early token} & \textbf{Middle token} & \textbf{Last token} \\ \midrule
\textbf{7b (14 layers)} & 0.77 $\pm$ 0.04 & 0.55 $\pm$ 0.07 & 0.79 $\pm$ 0.03 \\
\textbf{13b (16 layers)} & 0.83 $\pm$ 0.03 & 0.58 $\pm$ 0.06 & 0.81 $\pm$ 0.03 \\
\textbf{mistral (14 layers)} & 0.74 $\pm$ 0.02 & 0.54 $\pm$ 0.05 & 0.74 $\pm$ 0.02 \\
\textbf{phi3 (14 layers)} & 0.88 $\pm$ 0.03 & 0.56 $\pm$ 0.04 & 0.66 $\pm$ 0.03 \\ \bottomrule
\end{tabular}
\caption{AUROC of Task Generalization: 5 inst (3 categories) x 100 tasks}
\label{tab:task_generalization_tokens}
\end{table}


==> contents/table/transition_tokens.tex <==
% Inst generalization: Transition: first token(fp) → last token(fp) ratio

==> contents/why_llms_fail.tex <==
\section{Why do LLMs fail?: Hypothesis}\label{sec:why_fail}
\textcolor{red}{Include this section? Include it in introduction?}

Why do LLMs fail to follow instructions, even when those instructions are clear and familiar? Below, we examine three common hypotheses and explain why they do not fully account for the failures observed in our setting:

\textbf{Ambiguity}
A prevalent assumption is that instruction-following failures arise from ambiguous instructions. However, in our IFEval benchmark data, the instructions are meticulously designed to be clear and straightforward, leaving little room for misinterpretation. Despite this, LLMs still occasionally fail to follow these instructions, indicating that ambiguity is not the primary cause of the observed failures.

\textbf{Decoding Randomness}
Another potential explanation is the randomness inherent in the decoding process, which could lead to inconsistent outputs. In typical scenarios, sampling methods like temperature introduce variability, potentially causing the model to deviate from the expected response. However, in our experiments, we controlled for this by using deterministic decoding methods, such as greedy decoding, ensuring that randomness in decoding is not a contributing factor. Even with these controls in place, instruction-following failures persist, suggesting that the issue lies elsewhere.

\textbf{Instruction and Task Familiarity}
It might be expected that the model's familiarity with the instruction or task would play a role in its ability to follow instructions. One might assume that if an LLM has been trained on similar tasks or instructions, it would be more likely to succeed. However, our observations reveal inconsistencies that challenge this assumption. We encountered instances where the model successfully followed instructions in one case but failed in another, despite the tasks being similar and the instructions identical. This inconsistency indicates that familiarity alone does not fully explain the failures. \textcolor{red}{TODO: add example or explain more}


Given that ambiguity, decoding randomness, and familiarity do not fully account for why LLMs fail to follow instructions, we are left with a critical research question: Is there a difference in representation between success and failure cases in instruction-following? To address this, we analyzed the internal representations of LLMs during successful and unsuccessful instruction-following instances. Our goal was to determine if a specific dimension within the model’s representation space correlates with instruction-following success. If such a dimension exists, we hypothesize that by manipulating this dimension, we could shift failure cases into the success category, thereby demonstrating its significance in instruction adherence.



% These observations led us to explore other possible explanations. Our findings suggest that the key factor is how well the prompt is encoded within the model's input embeddings. Through our analysis, we identified a specific geometry related to instruction-following that is generalizable to unseen tasks, even when ambiguity and familiarity are controlled. This geometry within the input embedding space appears to play a crucial role in whether an LLM will successfully follow instructions.

% In summary, the success of instruction-following by LLMs depends not just on the clarity of the instructions, the familiarity of the task, or the absence of randomness in decoding, but critically on how effectively the prompt is encoded in the model’s internal representations. This insight shifts the focus from external factors to the internal processing mechanisms of the LLMs, providing a deeper understanding of the challenges in achieving reliable instruction-following.



% Why do LLMs fail to follow instructions, even when those instructions are clear and familiar? Several common explanations fall short:

% Ambiguity: The instructions in our benchmark data are clear and simple, ruling out ambiguity as a primary cause.
% Decoding Randomness: We controlled for randomness by not using sampling, so this cannot explain the failures.
% Instruction and Task Familiarity: We observed instances where LLMs succeeded with one example but failed with a similar task and identical instructions, indicating that familiarity alone is not the issue.
% Our findings suggest that the key factor is how well the prompt is encoded within the model's input embeddings. We identified a specific geometry related to instruction-following that is generalizable to unseen tasks, even when ambiguity and familiarity are controlled. This geometry explains why LLMs sometimes fail to follow instructions: the success of instruction-following depends on how effectively the prompt is encoded.



% Why do LLMs fail to follow instructions? Several factors have been proposed to explain this phenomenon, including ambiguous prompts, familiarity with the instructions, task complexity, and randomness in decoding. However, these factors alone do not fully explain the frequent failures in instruction-following, particularly in cases where instructions are clear and tasks are familiar to the model. Furthermore, in cases where sampling is not used, decoding randomness cannot be blamed for these failures.


% Then, why do LLMs fail to follow instructions? We can consider several hypotheses. First, is the instruction ambiguous? This isn't the case for the instruction-following benchmark data, where instructions are quite clear and simple. Second, is it due to randomness in decoding? We don't use sampling, so that's not the reason either. Next, how about familiarity with the instruction and task? Are they too difficult for LLMs to follow? We can observe cases with similar tasks and identical instructions where LLMs succeed in one example but fail in another.
% So, what else can explain why LLMs fail to follow instructions?

